CLR-Bench: Evaluating Large Language Models in College-level Reasoning

Large language models (LLMs) have demonstrated their remarkable performance across various language understanding tasks. While emerging benchmarks have been proposed to evaluate LLMs in various domains such as mathematics and computer science, they merely measure the accuracy in terms of the final prediction on multi-choice questions. However, it remains insufficient to verify the essential understanding of LLMs given a chosen choice. To fill this gap, we present CLR-Bench to comprehensively evaluate the LLMs in complex college-level reasoning. Specifically, (i) we prioritize 16 challenging college disciplines in computer science and artificial intelligence. The dataset contains 5 types of questions, while each question is associated with detailed explanations from experts. (ii) To quantify a fair evaluation of LLMs' reasoning ability, we formalize the criteria with two novel metrics. Q$\rightarrow$A is utilized to measure the performance of direct answer prediction, and Q$\rightarrow$AR effectively considers the joint ability to answer the question and provide rationale simultaneously. Extensive experiments are conducted with 40 LLMs over 1,018 discipline-specific questions. The results demonstrate the key insights that LLMs, even the best closed-source LLM, i.e., GPT-4 turbo, tend to `guess' the college-level answers. It shows a dramatic decrease in accuracy from 63.31% Q$\rightarrow$A to 39.00% Q$\rightarrow$AR, indicating an unsatisfactory reasoning ability.

==> tables/family.tex <==

\begin{table}[t]\footnotesize
	\centering
	\caption{\texttt{CLR-Bench} evaluation on different LLM families.}
	% \setlength{\tabcolsep}{3.3mm}
    \resizebox{0.5\linewidth}{!}{
	\begin{tabular}{clcc} 
	\toprule
	%\multirow{2}{*}{\textbf{\#}}&\multirow{2}{*}{\textbf{Models}} &\multicolumn{6}{c}{\textbf{Q$\rightarrow$A (Direct performance of prediction)}} &\multicolumn{7}{c}{\textbf{Q$\rightarrow$AR (Reasoning performance of rationale)}}\\
	%\cmidrule(lr){3-8} \cmidrule(lr){9-15}
    \textbf{\#} & \textbf{LLM Families} &\textbf{Q$\rightarrow$A}  &\textbf{Q$\rightarrow$AR} \\
    \midrule
    1 & claude-3-opus	& 62.57\%	& 38.56\%  \\
    2 &   claude-3-sonnet	& 60.51\%	& 38.51\% \\ 
    %\midrule
    %4 &   gemini-1.5-pro	& 71.62\%	& 78.34\%	& 55.38\%	& 46.67\%	& \underline{\textbf{52.42\%}}	& 60.36\%	& 50.46\%	& 40.54\%&	43.35\%	&50.24\%	& \underline{\textbf{12.83\%}}	& 37.21\% & 11 \\ 
    \midrule
    3 &  gpt-3.5-turbo	& 53.98\%	& 34.70\%  \\ 
    4 &  gpt-4-turbo	& \textcolor{purple}{\underline{\textbf{63.31\%}}}	& 39.00\% \\
    5 & gpt-4o	& 60.76\%	& 41.60\%  \\
    \midrule
    6 &  deepseek-chat	& 62.43\%	& \textcolor{purple}{\underline{\textbf{42.09\%}}} \\ 
    7 &  deepseek-7b-base-hf	& 40.08\%		& 20.73\%  \\
    8 &  deepseek-7b-chat	& 38.02\%	& 23.67\% \\
    \midrule
    9 &  gemma-7b-it	& 25.83\%		& 18.74\%  \\ 
    10 & gemma2-9b-hf 	& 16.26\%	& 8.77\% \\
    11 &  gemma2-9b-it	& 53.54\%	& 34.63\% \\
    \midrule
    12 &  llama-2-7b-chat & 35.07\%		& 21.32\% \\ 
    13 &  llama-2-7b-hf	 & 38.75\%	&  20.43\%  \\
    14 &  llama-3-8b-hf & 46.61\%	& 24.19\%  \\
    15 &  llama-3-8b-instruct	& 50.15\%	& 31.34\% \\
    16 & llama-3.1-8b-hf & 48.82\%	& 26.11\% \\ 
    17 &  llama-3.1-8b-instruct	&  50.49\%	& 29.54\%  \\
    18 &  llama-3.1-70b-hf		& 56.97\%		& 33.60\%  \\ 
    19 &  llama-3.1-70b-instruct	& 60.22\%	& 33.67\% \\
    20 & llama-3.2-1b-instruct	& 33.10\%		& 19.38\% \\ 
    21 &  llama-3.2-3b-instruct	& 43.37\%	& 28.36\% \\
    \midrule
    22 &  mistral-7b-instruct-v0.1		&  43.27\%	&  26.28\% \\
    23 &  mistral-7b-v0.1-hf & 48.18\%	& 26.33\% \\
    \midrule
    24 &  mixtral-8x7b-instruct-v0.1	& 41.36\% & 30.48\%  \\
    25 &  mixtral-8x7b-v0.1-hf	& 51.38\%	& 29.00\%  \\ 
    %\midrule
    %27 &  openchat-3.5	& 60.83\%	& 39.64\%	& 49.68\% &	25.71\%	& 36.25\%	& 44.94\%	& 26.01\% \\ 
    \midrule
    26 &  phi-3-mini-4k-instruct	& 53.78\%	& 35.56\% \\
    27 &  phi-3-medium-4k-instruct	& 57.12\%	& 37.60\% \\
    \midrule
    28 &   qwen1.5-7b-chat	& 26.67\%	& 22.35\%  \\ 
    29 &  qwen1.5-7b-hf	& 47.10\%	& 27.16\% \\ 
    30 & qwen2.5-7b-hf  & 54.62\%	& 33.37\%  \\
    31 &  qwen2.5-7b-instruct	&	56.93\%	& 37.25\% \\ 
    32 &  qwen2.5-32b-instruct	 & 63.31\%	& 42.29\%  \\ 
    33 &  qwen2.5-72b-hf	& 62.52\% & 37.89\% \\
    34 & qwen2.5-72b-instruct	& \textcolor{purple}{\underline{\textbf{64.05\%}}}	&  \textcolor{purple}{\underline{\textbf{40.79\%}}} \\
    \midrule
    35 &  yi-1.5-6b-chat	& 41.60\%	& 25.56\%  \\
    36 &  yi-1.5-6b-hf	& 48.08\% & 27.80\%  \\ 
    37 &  yi-1.5-34b-chat	& 52.95\%	& 33.87\%  \\
    38 &  yi-1.5-34b-hf	& 56.43\%	& 32.22\%  \\ 
    %28 & chatglm3-6b	& 3.23\%	& 48.65\%	& 18.67\%	& 10.48\%	& 10.78\%	& 15.72\%	& 4.61\%	& 2.70\% &	15.43\%	& 16.19\%	& 3.35\%	& 8.62\% & 41 \\ 
    \bottomrule
\end{tabular}}
\label{tab:family}
\end{table}

==> tables/main.tex <==

\begin{table*}[t]\footnotesize
	\centering
	\caption{\texttt{CLR-Bench} leaderboard of various models on the Q$\rightarrow$AR task. Each model is expected to answer correctly and rationalize accurately at the same time to get 1 point for each question.}
	% \setlength{\tabcolsep}{3.3mm}
    \resizebox{1\linewidth}{!}{
	\begin{tabular}{clcccccccccccc} 
	\toprule
	\multirow{2}{*}{\textbf{\#}}&\multirow{2}{*}{\textbf{Models}} &\multicolumn{6}{c}{\textbf{Q$\rightarrow$A (Direct performance of prediction)}} &\multicolumn{6}{c}{\textbf{Q$\rightarrow$AR (Reasoning performance of rationale)}}\\
	\cmidrule(lr){3-8} \cmidrule(lr){9-14}
	 & &\textbf{MC} &\textbf{MS} &\textbf{TF} &\textbf{FB} &\textbf{OE} &\textbf{Q$\rightarrow$A} &\textbf{MC} &\textbf{MS} &\textbf{TF} &\textbf{FB} &\textbf{OE} &\textbf{Q$\rightarrow$AR}  \\
	\midrule[0.6pt]
	1 & qwen2.5-7b-hf  & 69.12\%	& 54.95\%	& 54.11\% &	40.00\% &	49.07\%	& 54.62\%	& 43.55\%	& 34.46\% &	43.43\%	& 45.00\%	& 8.36\%	& 33.37\% \\
    2 &  gemma2-9b-it	& 72.81\% &	50.45\%	& 55.70\% &	43.81\%	& 40.52\%	& 53.54\%	& 45.62\%	& 32.88\%	& 47.15\%	& 44.52\%	& 7.90\%	& 34.63\% \\
    3 &  qwen2.5-72b-hf	& 80.18\%	& 73.42\%	& 60.44\% &	\underline{\textbf{47.62\%}}	& 52.04\%	& 62.52\%	& 50.00\%	& 43.02\%	& 45.97\%	& \underline{\textbf{49.52\%}}	& 11.99\%	& 37.89\% \\
    4 & gemma2-9b-hf & 16.13\%	& 47.75\%	& 11.71\%	& 9.52\%	& 11.34\%	& 16.26\%	& 11.29\%	& 8.33\%	& 10.60\%	& 11.67\%	& 3.62\%	& 8.77\% \\
    5 &  mixtral-8x7b-instruct-v0.1	& 59.91\%	& 45.05\%	& 34.18\%	& 16.19\%	& 43.12\%	& 41.36\% &	42.97\%	& 31.31\%	& 39.08\%	& 34.52\%	& 8.36\%	& 30.48\% \\
    6 &  phi-3-medium-4k-instruct	& 74.65\%	& 63.96\%	& 56.01\%	& 38.10\%	& 48.88\%	& 57.12\%	& 51.50\%	& 33.56\%	& 49.68\%	& 44.05\%	& 11.34\%	& 37.60\% \\
    7 & qwen2.5-72b-instruct	& \underline{\textbf{81.11\%}}	& \underline{\textbf{77.93\%}} &	\underline{\textbf{63.61\%}}	& 45.71\%	& \underline{\textbf{52.23\%}}	& \textcolor{purple}{\underline{\textbf{64.05\%}}}	& 50.58\% &	\underline{\textbf{45.50\%}}	& 53.56\%	& 48.10\%	& \underline{\textbf{13.10\%}}	& \textcolor{purple}{\underline{\textbf{40.79\%}}} \\
    8 &  llama-2-7b-hf	&  54.38\%	& 15.77\%	& 44.62\%	& 19.05\%	& 36.43\%	& 38.75\%	& 26.61\%	&  18.47\%	& 27.29\%	&  24.05\%	& 6.78\%	&  20.43\% \\
    9 &  llama-3.1-8b-instruct	&  63.13\%	& 51.80\% & 	56.96\%	& 25.71\%	& 41.82\%	&  50.49\%	& 39.06\% & 	22.97\%	& 41.85\%	&  33.57\%	& 8.55\%	& 29.54\% \\
    10 &  phi-3-mini-4k-instruct	& 69.12\%	& 59.46\%	& 55.38\%	& 34.29\%	& 44.80\%	& 53.78\%	& 49.42\% &	37.84\%	& 45.41\%	& 41.43\%	& 9.57\%	& 35.56\% \\
    11 &  yi-1.5-6b-chat	& 37.33\%	& 53.15\%	& 48.10\%	& 25.71\%	& 38.85\%	& 41.60\%	&30.30\%	&32.43\%	& 32.99\%	& 34.05\% &	6.88\%	& 25.56\% \\
    12 &  deepseek-7b-chat	& 49.31\%	& 27.48\%	&	45.57\%	&	20.00\%	&	31.41\%	& 38.02\%	&	30.76\% 	&	18.92\%	& 34.97\%	&	27.62\%		& 5.11\%		& 23.67\% \\
    13 &  yi-1.5-34b-chat	& 68.66\%	& 53.60\%	& 56.96\% &	40.95\%	& 39.96\%	& 52.95\%	& 40.90\% &	33.33\%	& 48.34\% &	44.76\%	& 7.16\%	& 33.87\% \\
    14 &  deepseek-7b-base-hf	& 49.77\%	& 36.49\%	& 44.94\%	& 18.10\%	& 36.62\%	& 40.08\%	& 27.88\% &	18.47\%	& 28.16\%	& 25.24\%	& 5.39\%	& 20.73\% \\
    15 &  llama-3.1-70b-instruct	& 80.18\%	& 74.77\%	& 61.39\%	& 40.00\%	& 44.61\%	& 60.22\%	& 44.24\% &	38.06\%	& 45.09\%	& 38.57\%	& 7.99\%	& 33.67\% \\
    16 &  llama-3-8b-hf	& 59.91\%	& 35.14\% &	50.95\%	& 26.67\% &	43.31\%	& 46.61\%	& 32.37\%	& 24.10\%	& 31.09\%	& 29.29\%	& 7.53\%	& 24.19\% \\
    17 &  mistral-7b-instruct-v0.1	&  57.60\%	&  45.05\%	& 40.82\%	&  21.90\%	&  42.19\%	&  43.27\%	&  35.48\%	&  27.48\%	&  34.41\%	&  33.33\%	& 6.04\%	&  26.28\% \\
    18 &  gemma-7b-it	& 15.21\%	& 37.84\%	& 45.25\% &	8.57\%	& 13.38\%	& 25.83\%	& 13.02\%	& 1.80\% &	35.52\%	& 20.24\%	& 10.04\%	& 18.74\% \\ 
    19 &   qwen1.5-7b-chat	& 32.26\%	& 50.00\%	& 11.71\%	& 13.33\%	& 35.32\%	& 26.67\%	& 27.42\% &	26.58\%	& 27.22\%	& 33.57\%	& 6.41\%	& 22.35\% \\ 
    20 &  yi-1.5-6b-hf	& 53.00\%	& 59.01\%	& 51.27\%	& 30.48\%	& 42.75\%	& 48.08\% &	33.53\%	& 29.95\%	& 39.16\%	& 35.00\%	& 6.13\%	& 27.80\% \\ 
    21 &  qwen2.5-32b-instruct	 & 80.18\%	& 75.23\% &	63.29\%	& 44.76\%	& 52.04\%	& 63.31\%	& \underline{\textbf{55.41\%}}	& \underline{\textbf{45.50\%}}	& \underline{\textbf{56.09\%}}	& 48.33\%	& 11.80\%	& 42.29\% \\ 
    22 &  qwen2.5-7b-instruct	& 70.97\%	& 63.06\% &	58.23\%	& 37.14\%	& 49.26\% &	56.93\%	& 52.65\%	& 34.23\% & 	50.32\%	& 41.90\%	& 8.92\%	& 37.25\% \\ 
    23 & llama-3.1-8b-hf &	62.67\%	& 40.54\%	& 51.58\% &	30.48\%	& 44.98\%	& 48.82\%	& 34.22\%	& 28.83\%	& 32.52\%	& 33.57\%	& 7.99\%	& 26.11\% \\ 
    24 &  llama-3.2-3b-instruct	& 57.14\%	& 39.19\%	& 49.05\%	& 23.81\%	& 34.94\%	& 43.37\%	& 40.55\%	& 21.40\%	& 38.29\%	& 32.62\%	& 8.09\%	& 28.36\% \\ 
    25 &  llama-3-8b-instruct	& 60.83\%	& 49.55\%	& 52.22\%	& 29.52\%	& 47.40\%	& 50.15\%	& 43.78\% &	26.35\%	& 41.30\%	& 36.19\%	& 9.76\%	& 31.34\% \\ 
    26 &  openchat-3.5	& 60.83\%	& 39.64\%	& 49.68\% &	25.71\%	& 36.25\%	& 44.94\%	& 35.94\%	& 22.75\%	& 33.86\%	& 30.24\%	& 8.46\%	& 26.01\% \\ 
    27 &  qwen1.5-7b-hf	& 58.99\%	& 54.50\%	& 47.15\%	& 37.14\%	& 38.29\%	& 47.10\%	& 36.64\%	& 33.11\%	& 32.99\%	& 35.95\%	& 6.78\%	& 27.16\% \\ 
    % 28 & chatglm3-6b	& 3.23\%	& 48.65\%	& 18.67\%	& 10.48\%	& 10.78\%	& 15.72\%	& 4.61\%	& 2.70\% &	15.43\%	& 16.19\%	& 3.35\%	& 8.62\% \\ 
    28 &  llama-2-7b-chat	& 38.25\%	& 36.49\%	& 39.24\%	& 13.33\%	& 35.50\%	& 35.07\%	& 26.04\%	 & 16.89\%	& 31.49\%	& 26.67\%	& 5.30\%	& 21.32\% \\ 
    29 &  mistral-7b-v0.1-hf &	58.06\%	& 42.79\%	& 50.63\%	& 37.14\%	& 43.87\%	& 48.18\%	& 33.06\%	& 29.05\%	& 34.10\%	& 35.24\%	& 7.16\%	& 26.33\% \\
    30 &  yi-1.5-34b-hf	& 70.97\%	& 58.11\% &	57.59\%	& 41.90\%	& 48.33\%	& 56.43\%	& 40.55\%	& 35.59\%	& 42.96\%	& 43.10\%	& 7.25\%	& 32.22\% \\ 
    31 &  mixtral-8x7b-v0.1-hf	& 67.28\%	& 39.64\%	& 53.48\% &	39.05\%	& 45.72\%	& 51.38\%	& 39.06\%	& 31.53\%	& 36.00\%	& 36.19\%	& 8.83\%	& 29.00\% \\ 
    32 &  llama-3.1-70b-hf	& 75.58\%	& 51.80\%	& 57.59\%	& 45.71\%	& 47.77\%	& 56.97\%	& 43.89\%	& 35.81\% &	41.46\%	& 45.48\%	& 10.50\%	& 33.60\% \\ 
    33 & llama-3.2-1b-instruct	& 41.47\%	& 40.99\% &	37.66\%	& 14.29\%	& 25.09\%	& 33.10\%	& 28.00\%	& 13.06\%	& 24.68\%	& 24.76\%	& 6.69\%	& 19.38\% \\ 
    \midrule
    34 &  gpt-3.5-turbo	& 66.67\%	& 63.13\%	& 58.54\% &	23.81\%	& 47.77\%	& 53.98\%	& 42.51\% &	41.22\%	& 49.60\%	& 39.29\%	& 6.41\%	& 34.70\% \\ 
    35 &   claude-3-sonnet	& 76.58\%	& 76.96\%	& 59.81\%	& 42.86\%	& 48.33\%	& 60.51\%	& 50.69\%	& 44.59\% &	48.26\%	& 45.95\%	& 11.80\%	& 38.51\%\\ 
    36 &   gemini-1.5-pro	& 71.62\%	& 78.34\%	& 55.38\%	& 46.67\%	& \underline{\textbf{52.42\%}}	& 60.36\%	& 50.46\%	& 40.54\%&	43.35\%	&50.24\%	& \underline{\textbf{12.83\%}}	& 37.21\% \\ 
    37 &  deepseek-chat	& 77.03\%	& 78.80\%	& 62.66\%	& 40.95\%	& 51.30\%	& 62.43\%	& \underline{\textbf{55.41\%}}	& 44.14\%	& 55.14\%	& 46.43\%	& 13.48\%	& \textcolor{purple}{\underline{\textbf{42.09\%}}} \\ 
    38 & gpt-4o	& 76.58\%	& \underline{\textbf{84.33\%}}	& \underline{\textbf{63.92\%}}	& \underline{\textbf{54.29\%}}	& 34.01\%	& 60.76\%	& 53.11\%	& 44.82\%	& \underline{\textbf{57.52\%}}	& \underline{\textbf{51.19\%}}	& 8.55\%	& 41.60\% \\
    49 &  gpt-4-turbo	& 78.38\%	& 82.49\%	& \underline{\textbf{63.92\%}}	& 50.48\%	& 45.91\%	& \textcolor{purple}{\underline{\textbf{63.31\%}}}	& 51.73\%	& 45.95\%	& 49.45\%	& 51.43\%	& 8.74\%	& 39.00\% \\
    40 & claude-3-opus-20240229	&  \underline{\textbf{81.53\%}}	& 80.18\%	& 62.66\%	& 52.38\%	& 44.42\%	& 62.57\%	& 50.35\%	& 43.02\%	& 50.08\%	& 50.00\%	& 9.20\%	& 38.56\% \\
    \bottomrule
	\end{tabular}}
\label{tab:main_Q_AR}
\end{table*}

==> tables/save.tex <==

\begin{table*}[t]\footnotesize
	\centering
	\caption{\texttt{CLR-Bench} leaderboard of various models on the Q$\rightarrow$AR task. Each model is expected to answer correctly and rationalize accurately at the same time to get 1 point for each question.}
	% \setlength{\tabcolsep}{3.3mm}
    \resizebox{1\linewidth}{!}{
	\begin{tabular}{clcccccccccccccc} 
	\toprule
	\multirow{2}{*}{\textbf{\#}}&\multirow{2}{*}{\textbf{Models}} &\multicolumn{6}{c}{\textbf{Q$\rightarrow$A (Direct performance of prediction)}} &\multicolumn{7}{c}{\textbf{Q$\rightarrow$AR (Reasoning performance of rationale)}}\\
	\cmidrule(lr){3-8} \cmidrule(lr){9-15}
    %\cmidrule(lr){3-9} \cmidrule(lr){10-16}
	 & &\textbf{MC} &\textbf{MS} &\textbf{TF} &\textbf{FB} &\textbf{OE} &\textbf{Q$\rightarrow$A} &\textbf{MC} &\textbf{MS} &\textbf{TF} &\textbf{FB} &\textbf{OE} &\textbf{Q$\rightarrow$AR} & \textbf{Rank} \\
    \midrule[0.6pt]
    %\multicolumn{16}{c}{\textbf{Close-Source LLMs}} \\
    %\midrule
    1 & claude-3-opus	&  \underline{\textbf{81.53\%}}	& 80.18\%	& 62.66\%	& 52.38\%	& 44.42\%	& 62.57\%	& 50.35\%	& 43.02\%	& 50.08\%	& 50.00\%	& 9.20\%	& 38.56\% & 6 \\
    2 &   claude-3-sonnet	& 76.58\%	& 76.96\%	& 59.81\%	& 42.86\%	& 48.33\%	& 60.51\%	& 50.69\%	& 44.59\% &	48.26\%	& 45.95\%	& 11.80\%	& 38.51\% & 7\\ 
    \midrule
    3 &  deepseek-chat	& 77.03\%	& 78.80\%	& 62.66\%	& 40.95\%	& 51.30\%	& 62.43\%	& \underline{\textbf{55.41\%}}	& 44.14\%	& 55.14\%	& 46.43\%	& 13.48\%	& \textcolor{purple}{\underline{\textbf{42.09\%}}} & 2\\ 
    4 &   gemini-1.5-pro	& 71.62\%	& 78.34\%	& 55.38\%	& 46.67\%	& \underline{\textbf{52.42\%}}	& 60.36\%	& 50.46\%	& 40.54\%&	43.35\%	&50.24\%	& \underline{\textbf{12.83\%}}	& 37.21\% & 11 \\ 
    \midrule
    5 &  gpt-3.5-turbo	& 66.67\%	& 63.13\%	& 58.54\% &	23.81\%	& 47.77\%	& 53.98\%	& 42.51\% &	41.22\%	& 49.60\%	& 39.29\%	& 6.41\%	& 34.70\% & 13 \\ 
    6 &  gpt-4-turbo	& 78.38\%	& 82.49\%	& \underline{\textbf{63.92\%}}	& 50.48\%	& 45.91\%	& \textcolor{purple}{\underline{\textbf{63.31\%}}}	& 51.73\%	& 45.95\%	& 49.45\%	& 51.43\%	& 8.74\%	& 39.00\% & 5\\
    7 & gpt-4o	& 76.58\%	& \underline{\textbf{84.33\%}}	& \underline{\textbf{63.92\%}}	& \underline{\textbf{54.29\%}}	& 34.01\%	& 60.76\%	& 53.11\%	& 44.82\%	& \underline{\textbf{57.52\%}}	& \underline{\textbf{51.19\%}}	& 8.55\%	& 41.60\% & 3 \\
    \midrule
    8 &  deepseek-7b-base-hf	& 49.77\%	& 36.49\%	& 44.94\%	& 18.10\%	& 36.62\%	& 40.08\%	& 27.88\% &	18.47\%	& 28.16\%	& 25.24\%	& 5.39\%	& 20.73\% & 36 \\
    9 &  deepseek-7b-chat	& 49.31\%	& 27.48\%	&	45.57\%	&	20.00\%	&	31.41\%	& 38.02\%	&	30.76\% 	&	18.92\%	& 34.97\%	&	27.62\%		& 5.11\%		& 23.67\% & 33 \\
    \midrule
    10 &  gemma-7b-it	& 15.21\%	& 37.84\%	& 45.25\% &	8.57\%	& 13.38\%	& 25.83\%	& 13.02\%	& 1.80\% &	35.52\%	& 20.24\%	& 10.04\%	& 18.74\% & 39 \\ 
    11 & gemma2-9b-hf & 16.13\%	& 47.75\%	& 11.71\%	& 9.52\%	& 11.34\%	& 16.26\%	& 11.29\%	& 8.33\%	& 10.60\%	& 11.67\%	& 3.62\%	& 8.77\% & 40\\
    12 &  gemma2-9b-it	& 72.81\% &	50.45\%	& 55.70\% &	43.81\%	& 40.52\%	& 53.54\%	& 45.62\%	& 32.88\%	& 47.15\%	& 44.52\%	& 7.90\%	& 34.63\% & 14\\
    \midrule
    13 &  llama-2-7b-chat	& 38.25\%	& 36.49\%	& 39.24\%	& 13.33\%	& 35.50\%	& 35.07\%	& 26.04\%	 & 16.89\%	& 31.49\%	& 26.67\%	& 5.30\%	& 21.32\% &  35\\ 
    14 &  llama-2-7b-hf	&  54.38\%	& 15.77\%	& 44.62\%	& 19.05\%	& 36.43\%	& 38.75\%	& 26.61\%	&  18.47\%	& 27.29\%	&  24.05\%	& 6.78\%	&  20.43\% & 37 \\
    15 &  llama-3-8b-hf	& 59.91\%	& 35.14\% &	50.95\%	& 26.67\% &	43.31\%	& 46.61\%	& 32.37\%	& 24.10\%	& 31.09\%	& 29.29\%	& 7.53\%	& 24.19\% & 32 \\
    16 &  llama-3-8b-instruct	& 60.83\%	& 49.55\%	& 52.22\%	& 29.52\%	& 47.40\%	& 50.15\%	& 43.78\% &	26.35\%	& 41.30\%	& 36.19\%	& 9.76\%	& 31.34\% & 20 \\
    17 & llama-3.1-8b-hf &	62.67\%	& 40.54\%	& 51.58\% &	30.48\%	& 44.98\%	& 48.82\%	& 34.22\%	& 28.83\%	& 32.52\%	& 33.57\%	& 7.99\%	& 26.11\% & 29 \\ 
    18 &  llama-3.1-8b-instruct	&  63.13\%	& 51.80\% & 	56.96\%	& 25.71\%	& 41.82\%	&  50.49\%	& 39.06\% & 	22.97\%	& 41.85\%	&  33.57\%	& 8.55\%	& 29.54\% & 22 \\
    19 &  llama-3.1-70b-hf	& 75.58\%	& 51.80\%	& 57.59\%	& 45.71\%	& 47.77\%	& 56.97\%	& 43.89\%	& 35.81\% &	41.46\%	& 45.48\%	& 10.50\%	& 33.60\% & 17 \\ 
    20 &  llama-3.1-70b-instruct	& 80.18\%	& 74.77\%	& 61.39\%	& 40.00\%	& 44.61\%	& 60.22\%	& 44.24\% &	38.06\%	& 45.09\%	& 38.57\%	& 7.99\%	& 33.67\% & 16 \\
    21 & llama-3.2-1b-instruct	& 41.47\%	& 40.99\% &	37.66\%	& 14.29\%	& 25.09\%	& 33.10\%	& 28.00\%	& 13.06\%	& 24.68\%	& 24.76\%	& 6.69\%	& 19.38\% & 38 \\ 
    22 &  llama-3.2-3b-instruct	& 57.14\%	& 39.19\%	& 49.05\%	& 23.81\%	& 34.94\%	& 43.37\%	& 40.55\%	& 21.40\%	& 38.29\%	& 32.62\%	& 8.09\%	& 28.36\% & 24 \\
    \midrule
    23 &  mistral-7b-instruct-v0.1	&  57.60\%	&  45.05\%	& 40.82\%	&  21.90\%	&  42.19\%	&  43.27\%	&  35.48\%	&  27.48\%	&  34.41\%	&  33.33\%	& 6.04\%	&  26.28\% & 28 \\
    24 &  mistral-7b-v0.1-hf &	58.06\%	& 42.79\%	& 50.63\%	& 37.14\%	& 43.87\%	& 48.18\%	& 33.06\%	& 29.05\%	& 34.10\%	& 35.24\%	& 7.16\%	& 26.33\% & 27 \\
    \midrule
    25 &  mixtral-8x7b-instruct-v0.1	& 59.91\%	& 45.05\%	& 34.18\%	& 16.19\%	& 43.12\%	& 41.36\% &	42.97\%	& 31.31\%	& 39.08\%	& 34.52\%	& 8.36\%	& 30.48\% & 21 \\
    26 &  mixtral-8x7b-v0.1-hf	& 67.28\%	& 39.64\%	& 53.48\% &	39.05\%	& 45.72\%	& 51.38\%	& 39.06\%	& 31.53\%	& 36.00\%	& 36.19\%	& 8.83\%	& 29.00\% & 23 \\ 
    \midrule
    27 &  openchat-3.5	& 60.83\%	& 39.64\%	& 49.68\% &	25.71\%	& 36.25\%	& 44.94\%	& 35.94\%	& 22.75\%	& 33.86\%	& 30.24\%	& 8.46\%	& 26.01\% & 30 \\ 
    \midrule
    28 &  phi-3-mini-4k-instruct	& 69.12\%	& 59.46\%	& 55.38\%	& 34.29\%	& 44.80\%	& 53.78\%	& 49.42\% &	37.84\%	& 45.41\%	& 41.43\%	& 9.57\%	& 35.56\% & 12\\
    29 &  phi-3-medium-4k-instruct	& 74.65\%	& 63.96\%	& 56.01\%	& 38.10\%	& 48.88\%	& 57.12\%	& 51.50\%	& 33.56\%	& 49.68\%	& 44.05\%	& 11.34\%	& 37.60\% & 9\\
    \midrule
    30 &   qwen1.5-7b-chat	& 32.26\%	& 50.00\%	& 11.71\%	& 13.33\%	& 35.32\%	& 26.67\%	& 27.42\% &	26.58\%	& 27.22\%	& 33.57\%	& 6.41\%	& 22.35\% & 34 \\ 
    31 &  qwen1.5-7b-hf	& 58.99\%	& 54.50\%	& 47.15\%	& 37.14\%	& 38.29\%	& 47.10\%	& 36.64\%	& 33.11\%	& 32.99\%	& 35.95\%	& 6.78\%	& 27.16\% & 26 \\ 
    32 & qwen2.5-7b-hf  & 69.12\%	& 54.95\%	& 54.11\% &	40.00\% &	49.07\%	& 54.62\%	& 43.55\%	& 34.46\% &	43.43\%	& 45.00\%	& 8.36\%	& 33.37\% & 18 \\
    33 &  qwen2.5-7b-instruct	& 70.97\%	& 63.06\% &	58.23\%	& 37.14\%	& 49.26\% &	56.93\%	& 52.65\%	& 34.23\% & 	50.32\%	& 41.90\%	& 8.92\%	& 37.25\% & 10 \\ 
    34 &  qwen2.5-32b-instruct	 & 80.18\%	& 75.23\% &	63.29\%	& 44.76\%	& 52.04\%	& 63.31\%	& \underline{\textbf{55.41\%}}	& \underline{\textbf{45.50\%}}	& \underline{\textbf{56.09\%}}	& 48.33\%	& 11.80\%	& 42.29\% & \textcolor{red}{\textbf{1}} \\ 
    35 &  qwen2.5-72b-hf	& 80.18\%	& 73.42\%	& 60.44\% &	\underline{\textbf{47.62\%}}	& 52.04\%	& 62.52\%	& 50.00\%	& 43.02\%	& 45.97\%	& \underline{\textbf{49.52\%}}	& 11.99\%	& 37.89\% & 8\\
    36 & qwen2.5-72b-instruct	& \underline{\textbf{81.11\%}}	& \underline{\textbf{77.93\%}} &	\underline{\textbf{63.61\%}}	& 45.71\%	& \underline{\textbf{52.23\%}}	& \textcolor{purple}{\underline{\textbf{64.05\%}}}	& 50.58\% &	\underline{\textbf{45.50\%}}	& 53.56\%	& 48.10\%	& \underline{\textbf{13.10\%}}	& \textcolor{purple}{\underline{\textbf{40.79\%}}} & 4\\
    \midrule
    37 &  yi-1.5-6b-chat	& 37.33\%	& 53.15\%	& 48.10\%	& 25.71\%	& 38.85\%	& 41.60\%	&30.30\%	&32.43\%	& 32.99\%	& 34.05\% &	6.88\%	& 25.56\% & 31 \\
    38 &  yi-1.5-6b-hf	& 53.00\%	& 59.01\%	& 51.27\%	& 30.48\%	& 42.75\%	& 48.08\% &	33.53\%	& 29.95\%	& 39.16\%	& 35.00\%	& 6.13\%	& 27.80\% & 25 \\ 
    39 &  yi-1.5-34b-chat	& 68.66\%	& 53.60\%	& 56.96\% &	40.95\%	& 39.96\%	& 52.95\%	& 40.90\% &	33.33\%	& 48.34\% &	44.76\%	& 7.16\%	& 33.87\% & 15 \\
    40 &  yi-1.5-34b-hf	& 70.97\%	& 58.11\% &	57.59\%	& 41.90\%	& 48.33\%	& 56.43\%	& 40.55\%	& 35.59\%	& 42.96\%	& 43.10\%	& 7.25\%	& 32.22\% & 19 \\ 
    %28 & chatglm3-6b	& 3.23\%	& 48.65\%	& 18.67\%	& 10.48\%	& 10.78\%	& 15.72\%	& 4.61\%	& 2.70\% &	15.43\%	& 16.19\%	& 3.35\%	& 8.62\% & 41 \\ 
    \bottomrule
\end{tabular}}
\label{tab:family}
\end{table*}
